Zero-shot racially balanced dataset generation using an existing biased StyleGAN2

Facial recognition systems have made significant strides thanks to data-heavy deep learning models, but these models rely on large privacy-sensitive datasets. Further, many of these datasets lack diversity in terms of ethnicity and demographics, which can lead to biased models that can have serious societal and security implications. To address these issues, we propose a methodology that leverages the biased generative model StyleGAN2 to create demographically diverse images of synthetic individuals. The synthetic dataset is created using a novel evolutionary search algorithm that targets specific demographic groups. By training face recognition models with the resulting balanced dataset containing 50,000 identities per race (13.5 million images in total), we can improve their performance and minimize biases that might have been present in a model trained on a real dataset.

==> sections/intro.tex <==



Facial recognition systems that traditionally made use of handcrafted features have achieved human-level performance with the help of deep learning models. This shift saw the collection of large amounts of privacy-sensitive datasets for the purpose of training these large models. This process of data collection is not only expensive but has various other issues. Firstly, these large datasets often exhibit a lack of ethnic and demographic diversity, leading the deep facial recognition models to suffer from similar biases across various settings. Ensuring the collection of highly diverse image datasets is difficult and expensive. Secondly, various countries \cite{us-bill, india_supreme, de2018guide} have recognized biometric data privacy as a fundamental right, and thus regulating its collection and usage by law. This makes it even more difficult to collect data from a large number of user and it also raises privacy concerns. Various public available dataset have already been retracted due to these issues \cite{}. 



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{generated_imgs.png}
    \caption{Examples of images generated for different ethnicities using our approach.}
    \label{fig:examples }
\end{figure}


Thus to deal with these issues this work presents an approach to build fairer facial recognition models making use of the advancements in image generation. As compared to manual data collection and annotation, generative models provide a cost and time-effective alternative. Generative models allow for better control of the settings, such as different environmental conditions, lighting, occlusions, camera angle, and background making it possible to train models that are more robust and adaptable. Additionally, in contrast to real data, synthetically generated datasets do not contain any personally identifiable information. They look similar to the real data that they were trained on but provide crucial privacy protection.


However, this is not as simple as existing generative models as highly biased. In fact, when randomly sampling 10,000 samples from a stylegan2 model, only 26 corresponded to Indians, 171 to Africans and in contrast over 6500 were that for White people. This makes simple rejection sampling not only inefficient but also implausible for generating a large number of samples for the underrepresented groups. 


Given the biased nature of existing generative models, previous methods that have looked at data generation for specific protected attributes have generally trained a generative model from scratch or finetuned an existing model. Each of these processes requires the collection of a large amount of real data for the target protected attribute. For example a recent work, \cite{sevastopolsky2022boost} collected over 5M images of Africans and 3M images of Asians from various YouTube sources. 

In contrast, as we show there is significant variability in already existing generative models that can be exploited. Moreover, previous research has shown the existence of latent directions or high dimensional latent spaces that correspond to different facial or protected attributes \cite{}. In this regard, we propose a simple search-based algorithm that in a one-shot manner can generate a large number of synthetic identities. In this study, we generate over 50,000 distinct synthetic identities for six different racial groups - Indian, White, African, Black, Asian, Middle Eastern, and Latino Hispanic. Thus, in total, we generate 13.5 million images with 45 images per person. 


Finally, we show that pretraining on this large corpus of balanced data can boost the performance of facial recognition systems. We show results for three different facial recognition systems namely ArcFace \cite{deng2019arcface}, AdaFace \cite{kim2022adaface}, and ElasticFace \cite{boutros2022elasticface}. There are significant improvements over models trained using widely accepted unbalanced datasets such as VGGFace2 \cite{cao2018vggface2}. We show improvements even on the BUPT balanced-face dataset \cite{wang2020mitigating} which contains an equal number of identities per race. 

Furthermore, this approach of generating a balanced dataset from a biased generative model can be used for numerous downstream tasks such as ethnicity classification, and, age classification. We only show results for generating balanced racial identities but this approach can just as easily be applied to other protected attributes such as age and gender. 



We make the following contributions in this paper:
\begin{itemize}
    \item We propose a simple evolutionary search-based approach to generate a large balanced set of images using an existing biased generative model. Our approach doesn't require any training or finetuning of the generative model. 
    \item We conduct experimental studies to show that training facial recognition models on this generated data with some finetuning on real data can boost the performance of these models. Especially in cases when the real image training set is biased. 
\end{itemize}



==> sections/results.tex <==






